Is a Good Representation Sufficient for Sample Efficient Reinforcement Learning?

Modern deep learning methods provide effective means to learn good representations. However, is a good representation itself sufficient for sample efficient reinforcement learning? This question has largely been studied only with respect to (worst-case) approximation error, in the more classical approximate dynamic programming literature. With regards to the statistical viewpoint, this question is largely unexplored, and the extant body of literature mainly focuses on conditions which permit sample efficient reinforcement learning with little understanding of what are necessary conditions for efficient reinforcement learning. This work shows that, from the statistical viewpoint, the situation is far subtler than suggested by the more traditional approximation viewpoint, where the requirements on the representation that suffice for sample efficient RL are even more stringent. Our main results provide sharp thresholds for reinforcement learning methods, showing that there are hard limitations on what constitutes good function approximation (in terms of the dimensionality of the representation), where we focus on natural representational conditions relevant to value-based, model-based, and policy-based learning. These lower bounds highlight that having a good (value-based, model-based, or policy-based) representation in and of itself is insufficient for efficient reinforcement learning, unless the quality of this approximation passes certain hard thresholds. Furthermore, our lower bounds also imply exponential separations on the sample complexity between 1) value-based learning with perfect representation and value-based learning with a good-but-not-perfect representation, 2) value-based learning and policy-based learning, 3) policy-based learning and supervised learning and 4) reinforcement learning and imitation learning.

==> algorithm.tex <==
\begin{algorithm}[t]
	\caption{Check}
	\begin{algorithmic}[1]
		\State \textbf{Input: $s,h$}
		%		\State If $\exists a^* \in \actions$: such that\begin{align*}
		%			\min_{\theta \in \Theta_h} \langle \theta, \phi(s,a^*)\rangle \ge \max_{a \in \actions - \left\{a^*\right\}} \max_{\theta \in \Theta_h} \langle \theta, \phi(s,a)\rangle,
		%		\end{align*}
		%		\textbf{Return} $a^*.$
		\State \textbf{Return} an action subset $\hat{\actions} \subset \actions$ that satisfies for any $\hat{a} \in \hat{\actions}$\begin{align*}
		\max_{f \in \fclass_h} f\left(s,\hat{a}\right) \ge \max_{a \in \actions} \min_{f \in \fclass_h} f\left(s,a\right)
		\end{align*}
	\end{algorithmic}
	\label{algo:check}
\end{algorithm}



\begin{algorithm}[t]
	\caption{Explore}
	\begin{algorithmic}[1]
		\State \textbf{Input}: $s,h$.
		\For{$a \in $ Check ($s,h$)}
		\State Let $s'$ be the state from the state $s$ taking action $a$.
		\State Add $(s,a,r(s,a)+Explore(s',h+1))$ to $D_h$.
		\EndFor
		\State \textbf{Return:} $\max_{a \in \text{Check ($s,h$)}} (s,a,r(s,a)+Explore(s',h+1))$. 
	\end{algorithmic}
	\label{algo:explore}
\end{algorithm}

\begin{algorithm}[t]
	\caption{Policy Based Learning with Function Approximation for Deterministic Systems}
	\begin{algorithmic}[1]   
		\State Explore ($s_0$).
		\State Execute optimal policy according to $\fclass_1,\ldots,\fclass_H$.
		%\State $D_{a}^h$: set of $\phi(s)$ that we execute action $a$. Each element in $D_{a}^h$ corresponds to one element in $Y_{a}^h$ (initialized as an empty set).
	\end{algorithmic}
	\label{algo:main}
\end{algorithm}

In this section we propose a general framework for policy-based learning with function approximation in the deterministic setting.
We maintain a dataset $D_h = \left\{(s_h^i,a_h^i,q_h^i)\right\}$ for each level $h \in [H]$ where $q_h^i$ represents the $Q$-value of $(s_h^i,a_h^i)$.
Note $D_h$ implies constrains on the feasible parameter space.
We let $\fclass_1,\ldots,\fclass_H$ denote the current feasible policy set.
$\fclass_h$ satisfies that any $f \in \fclass_h$ we have that for any pair $(s_h^i,a_h^i,q_h^i), (s_h^j,a_h^j,q_h^j)$ with $q_h^i > q_h^j$:\begin{align}
	f\left(s_h^i,a_h^i\right) > f\left(s_h^j,a_h^j\right). \label{eqn:consistent}
\end{align}
Depending on the assumptions, there may be other consistent assumptions which we will talk about later in specific examples.

The algorithm is based on recursion.
At any state, we first check what are the possible actions that can possibly be optimal and we just try all possibly optimal actions.
During exploration, we also add the optimal $Q$-value for each state-action pair we visit.
At last we can just execute optimally according to $\Theta_1,\ldots,\Theta_H$.
We remark that generalization to noisy reward with the gap assumption is almost trivial as we can just visit the same state many times and make the noise smaller than the gap.
See Algorithm~\ref{algo:check}-\ref{algo:main} for pseudo-codes.






Now we discuss concrete sample complexity bounds for specific instances.
From the algorithm, it is clear that we only need to bound that number of times $\abs{\hat{\actions}} > 1$.

\begin{example}[Whole Space]
	\label{example:epsnet}
Without loss of generality, suppose $\phi(\cdot,\cdot)$ is on the unit sphere and $\Theta_h$ is a subset of the unit sphere.
Suppose we know the linear predictor has a margin $\gamma$.
Then the sample complexity is $O\left(\left(\frac{1}{\gamma}\right)^d\right)$.
This can be proved by the covering argument.

\end{example}

\begin{example}[Cluster-able Setting]
	\label{example:clustering}
Consider the following setting. 
At each level $h \in [H]$ and $a \in \actions$, let $\states_h^a$ be the set of states such that $a$ is the optimal action.
For any $s \in \states_h^a$ and $s' \in \states_h^{a'}$, we assume $\norm{\phi(s) - \phi(s')} \ge \gamma$, i.e., the cluster distance is larger than $\gamma$.
We also assume for any $s_1,s_2 \in \states_h^a$, $\norm{\phi(s)-\phi(s')} \le \frac{\gamma}{2}.$\footnote{Here we only need a feature map for states.}
Note in this setting, whenever we identify a state's optimal action, we identify all states that share the same action, so the sample complexity is just $\poly(N_{cluster},\actions,\frac{1}{\gamma})$ where $N_{cluster}$ is the number of clusters.
We can generalize this setting to multiple (but finite) clusters per action.
\end{example}

\begin{example}[Finite Policy Set]
\label{example:polynomial_set}
Assuming $\fclass_1,\ldots,\fclass_H$ are all finite.
Note since we have horizon $H$, the total number of unstationary policy is $\Pi_{h=1}^H \abs{\fclass_h}$.
Consider one trajectory in our algorithm.
Let $h$ be the last level that $\abs{\hat{\actions}} \ge 2$.
After the trajectory, we at least get rid of one policy from $\fclass_h$.
Therefore, in total we only need $\sum_{h=1}^H \abs{\fclass_h}$ trajectories.
\end{example}

\begin{example}[State Aggregation / Tabular]
\label{example:state_aggregation}
Note one can view tabular case and state aggreation as special cases in cluster-able setting as the diameter is $0$. 
\end{example}

\begin{example}[$Q$-learning]
\label{example:q_learning}
Suppose we know the optimal $Q^*$ is a linear function.
We know if $f \in \fclass$, it also satisfies $f(s_h^i,a_h^i) = q_h^i$ for all $i \in D_h$.
Note using $d$ samples, we can identify one linear function with $d$ coordinates, so the we at most need $Hd$ trajectories.
We recover the result in \cite{wen2013efficient,du2019qlearning}.
\end{example}

Basically we can provide either polynomial upper bound or an exponential lower bound for the setting considered in \cite{wen2013efficient}.









==> model_based.tex <==
%%\subsection{Lower Bound for Model-based Learning}\label{sec:lb_model}
%Here we present our lower bound for model-based learning.
%Recently, \citet{yang2019sample} proposed the linear transition assumption which was later studied in~\citet{yang2019reinforcement, jin2019provably}.
%Under this assumption, \citet{yang2019sample, yang2019reinforcement, jin2019provably} developed algorithms with polynomial sample complexity.
%Again, we assume the agent is given a feature extractor $\phi: \states \times \actions \to \mathbb{R}^d$, and now we state the assumption formally as follow.
%\begin{asmp}[Approximate Linear MDP]
%	\label{asmp:linear_trans}
%	There exists $\approxerr > 0$, $\beta_0, \beta_1, \ldots, \beta_{H - 1} \in \mathbb{R}^d$ and $\psi : \states \to \mathbb{R}^d$ such that for any $h \in [H - 1]$, $\left(s,a\right) \in \states_h \times \actions$ and $s' \in \states_{h + 1}$, 
%	%	\begin{align}
%	$\abs{\trans\left(s' \mid s,a\right) - \langle \psi(s'), \phi\left(s,a\right) \rangle} \le \approxerr$ and $\abs{\E[R(s,a)] - \left\langle\beta_h, \phi(s,a)\right\rangle} \le \approxerr$.
%	% \label{eqn:q_star_linear}
%	%	\end{align}
%\end{asmp}
%It has been shown in \citet{yang2019sample, yang2019reinforcement, jin2019provably} if $\| \trans\left( \cdot \mid s, a\right) - \langle \psi(\cdot), \phi\left(s,a\right) \rangle \|_1$ is bounded, then the problem admits an algorithm with polynomial sample complexity.
%Now we show that when $\approxerr = \Omega\left(\sqrt{\frac{H}{d}}\right)$ in Assumption~\ref{asmp:linear_trans}, the agent needs exponential number of samples to find a near-optimal policy.
%\begin{thm}[Exponential Lower Bound for Linear Transition Model]
%	\label{thm:lb_transition}
%	There exists a family of MDPs and a feature extractor $\phi$ that satisfy Assumption~\ref{asmp:linear_trans} with $d = 2 \cdot \lceil 8 \ln 2 H / \approxerr^2 \rceil$, such that any algorithm that returns a $1/2$-optimal policy with probability $0.9$ needs to sample $\Omega\left(2^{H}\right)$ trajectories.
%%	For the family of MDPs and feature map $\phi\left(\cdot,\cdot\right)$ in Theorem~\ref{thm:lb_q_all}, Assumption~\ref{asmp:q_all_linear} is satisfied with $\approxerr = \varepsilon$.
%	\end{thm}
%Recall that for the family of MDPs in Theorem~\ref{thm:lb_q_all}, the agent needs exponential number of samples to find a near-optimal policy. 
%Thus, Theorem~\ref{thm:lb_transition} in fact implies that under Assumption~\ref{asmp:linear_trans} with $\approxerr = \Omega\left(\sqrt{\frac{H}{d}}\right)$, the exponential sample complexity lower bound still holds.



==> proof_ideas_old.tex <==
\paragraph{The binary tree hard instance. } All our lower bound are proved based on reductions from the following binary tree hard instance.
In the binary tree hard instance, both the transition $\trans$ and the reward $R$ are deterministic. 
There are $H$ levels of states, which form a full binary tree of depth $H$.
There are $2^{h - 1}$ states in level $h$, and thus $2^{H} - 1$ states in total.
Among all the $2^{H - 1}$ leaves in level $H$, there is only one state with reward $R = 1$, and for all other states in the MDP, the corresponding reward value $R = 0$.
Intuitively, to find a $0.99$-optimal policy for such MDPs, the agent must enumerate all possible states in the level $H$ to find the state with reward $R = 1$.
Doing so intrinsically induces a sample complexity of $\Omega(2^H)$.
This intuition is formalized in Theorem~\ref{thm:indq} using Yao's minimax principle~\citep{yao1977probabilistic}.
\ruosong{TODO: Unify name for suboptimal policy.}

\paragraph{Lower bound for value-based learning and model-based learning.}
We now show how to construct a set of features so that Assumption~\ref{asmp:q_star_linear}-\ref{asmp:linear_trans} hold.
Our main idea is to the utilize the following fact regarding the identity matrix: $\varepsilon$-$\mathrm{rank}(I_{2^H}) \le O(H / \varepsilon^2)$.
Here for a matrix $A \in \mathbb{R}^{n \times n}$, its {\em $\varepsilon$-$\mathrm{rank}$} (a.k.a {\em approximate rank}) is defined to be $\min \{ \mathrm{rank}(B): B \in \mathbb{R}^{n \times n}, \|A - B\|_{\infty} \le \varepsilon \}$,
where we use $\|\cdot\|_{\infty}$ to denote the entry-wise $\ell_{\infty}$ norm of a matrix. 
The upper bound $\varepsilon$-$\mathrm{rank}(I_{n}) \le O(\log n / \varepsilon^2)$ was first proved in~\cite{alon2009perturbed} using the Johnson-Lindenstrauss Lemma~\citep{johnson1984extensions}, and we also provide a proof for completeness in Lemma~\ref{lem:jl}.
\textbf{
The concept of $\varepsilon$-$\mathrm{rank}$ has wide applications in theoretical computer science~\citep{alon2009perturbed, barak2011rank, alon2013approximate, alon2014cover, chen2019classical}, but to our best knowledge, this is the first time that it appears in reinforcement learning.
\ruosong{Maybe move this to related work.}}
This fact can be alternatively stated as follow: there exists $\Phi \in \mathbb{R}^{2^H \times O(H / \varepsilon^2)}$ such that $\|I_{2^H} - \Phi \Phi^{\top}\|_{\infty} \le \varepsilon$.
We interpret each row of $\Phi$ as the feature of a state in the binary tree. 
By construction of $\Phi$, now the features of states in the binary tree have a nice property that (i) each feature vector has approximately unit norm and (ii) different feature vector are nearly orthogonal. 
Using this set of features, we can now show that Assumption~\ref{asmp:q_star_linear}-\ref{asmp:linear_trans} hold.
Here we prove Assumption~\ref{asmp:q_star_linear} holds as an example, and prove other assumptions also hold in the appendix.

To prove Assumption~\ref{asmp:q_star_linear}, we note that in the binary tree hard instance, for each level $h$, only a single state satisfies $Q^* = 1$, and all other states satisfy $Q^* = 0$. We simply take $\theta_h$ to be the feature of the state with $Q^* = 1$. 
Since all feature vectors are nearly orthogonal, Assumption~\ref{asmp:q_star_linear} holds.

Since the above fact regarding the identity matrix can be proved by simply taking each row of $\Phi$ to be a random unit vector, our lower bound reveals another intriguing (yet disappointing) aspect of Assumption~\ref{asmp:q_star_linear}: for the binary tree instance, almost all feature maps induce a hard MDP instance.
This again suggests that a good representation itself may not necessarily lead to efficient reinforcement learning and additional assumptions (e.g. on the reward distribution) could be crucial. 

\paragraph{Lower bound for policy-based learning.} It is easy to construct a set of feature vectors for the binary tree instance so that Assumption~\ref{asmp:linear_policy_realizable} holds, even if $d = 1$. 
We simply set $\phi(s, a)$ to be $+1$ if $a = a_1$ and $-1$ if $a = a_2$.
For each level $h$, for the unique state $s$ in level $h$ with $Q^* = 1$, we set $\theta_h$ to be $1$ if $\pi^*(s) = a_1$ and $-1$ if $\pi^*(s) = a_2$.
It is easy to verify that Assumption~\ref{asmp:linear_policy_realizable} indeed holds for this set of feature.

To prove that the lower bound still holds even under Assumption~\ref{asmp:linear_policy_margin}, we slightly change the reward function of states in level $H$ in the binary tree instance so that there exists a unique optimal action for each state in the MDP. 
See Figure~\ref{fig:tree_policy} for an example with $H = 3$ levels of states.
Another nice property of the reward function is that for all states $s$ we always have $\pi^*(s) = a_1$.
Now, in order to prove the lower bound, for each state in level $H$, we change its original reward to $1$, so that we define $2^{H - 1}$ different new MDPs.
An exponential sample complexity lower bound can be proved using the same argument as the original binary tree hard instance, and now we show this set of MDPs satisfy Assumption~\ref{asmp:linear_policy_margin}.

To define features for the states, we first show in Lemma~\ref{lem:geo} that there exists a set $\mathcal{N} \subseteq \mathbb{S}^{d - 1}$ with $|\mathcal{N}| = (1 / \triangle)^{\Omega(d)}$, so that for each $p \in \mathcal{N}$, there exists a hyperplane $L$ that separates $p$ and $\mathcal{N} \setminus \{p\}$, and all vectors in $\mathcal{N}$ have distance at least $\triangle$ to $L$. 
Equivalently, for each $p \in \mathcal{N}, $we can always define a linear function $f_p$ so that $f_p(p) \ge \triangle$ and $f_p(q) \le -\triangle$ for all $q \in \mathcal{N} \setminus \{p\}$.
This can be proved using standard lower bounds on the size of $\varepsilon$-nets.
Now we simply use vectors in $\mathcal{N}$ as features of states. 
By construction of the reward function, for each level $h$, there could only be two possible cases for the optimal policy $\pi^*$.
I.e., either $\pi^*(s) = a_1$ for all states in level $h$, or $\pi^*(s) = a_2$ for a unique state $s$ and $\pi^*(s') = a_1$ for all $s \neq s'$.
In both cases, we can easily define a linear function with margin $\triangle$ to implement the optimal policy $\pi^*$, and thus Assumption~\ref{asmp:linear_policy_margin} holds.

Notice that in the proof of the second lower bound, we critically relies on $d = \Theta(H)$, so that we can utilize the curse of dimensionality to construct a large set of vectors as features.
